Two-Step SPLADE: Simple, Efficient and Effective Approximation of SPLADE

Learned sparse models such as SPLADE have successfully shown how to incorporate the benefits of state-of-the-art neural information retrieval models into the classical inverted index data structure. Despite their improvements in effectiveness, learned sparse models are not as efficient as classical sparse model such as BM25. The problem has been investigated and addressed by recently developed strategies, such as guided traversal query processing and static pruning, with different degrees of success on in-domain and out-of-domain datasets. In this work, we propose a new query processing strategy for SPLADE based on a two-step cascade. The first step uses a pruned and reweighted version of the SPLADE sparse vectors, and the second step uses the original SPLADE vectors to re-score a sample of documents retrieved in the first stage. Our extensive experiments, performed on 30 different in-domain and out-of-domain datasets, show that our proposed strategy is able to improve mean and tail response times over the original single-stage SPLADE processing by up to $30\times$ and $40\times$, respectively, for in-domain datasets, and by 12x to 25x, for mean response on out-of-domain datasets, while not incurring in statistical significant difference in 60\% of datasets.

==> arxiv.tex <==
\section{Introduction}

Given our recent results and other articles in the literature, the most significant way to improve the latency of SPLADE models has been to reduce the number of query terms, followed by some distance by the pruning of document terms. However, when we approach very fast models ($\approx$ BM25 latency) we start noticing a sharp drop in effectiveness, especially in out-of-domain experiments. We provide empirical evidence in Table~\ref{tab:summary}.

\input{tables/summary.tex}

One way to counter-act this is to limit the number of documents searched with the expanded query terms. To do so, we split our first-stage ranking into two steps: i) in the first stage we prune aggressively so that both queries and documents have statistics similar to a non expanded dataset\footnote{For example, on MSMARCO we limit ourselves to 5 tokens per query and 32 per document} and return a top-$k$; and ii) rerank the top-$k$ using the full documents and queries from SPLADE. For now we always consider the same SPLADE model for both steps, but this could be improved by using two different models (although with increased latency due to paying the query encoding twice).

\section{Method}

In order to achieve the best of both worlds: i) Fast retrieval; and ii) Accurate out-of-domain effectiveness, we aim to combine our methods. The main goal is that for most documents we perform very simple and fast computations (See IDs 1 and 2 which describe exactly how to get those faster SPLADE implementations) and then after getting a small set of candidates (around 100) we allow the system to perform slightly more costly computation. This is indeed how most systems are implemented, with a ``first-stage`` and ''second-stage`` retrieval, where most of the time the first-stage is a vector-based retrieval and the second stage a cross-encoder. While SPLADE mostly belongs to the first-stage, there's nothing that obliges it to perform retrieval in a single step. So we actually propose to split the retrieval, with the first stage being a very rough representation of the representations (aggressive document and query pruning) and the second stage using the actual representation.\footnote{Maybe we could imagine a residual system later?} We describe this algorithm in Algorithm~\ref{alg:pruning} (Preprocessing) and Algorithm~\ref{alg:query} (Two stage processing).

\begin{algorithm}
\caption{Preprocessing: Pruning models}\label{alg:pruning}
\begin{algorithmic}[1]
\Require{$T$ collection, $Q$ collection, preprocessed for SPLADE}
\State Compute averages of $T$ and $Q$ and store as $l_d$ and $l_q$
\State \textbf{Initialize} $I^1$ as an empty index // Pruned document index
\State \textbf{Initialize} $I^2$ as an empty index // Full document index
\For{each document $d$ in $T$}
    \State $d' = $Prune $d$ to size $l_d$ by selecting the highest values
    \State Add $d'$ to $I^1$
    \State Add $d$ to $I^2$
    
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Two stage Processing Algorithm}\label{alg:query}
\begin{algorithmic}[1]
\Require{Indexes $I^1$ and $I^2$, a query $q$, an average query size $l_q$ and the amount of documents to return $k$}
    \State $q' = $Prune $q$ to size $l_q$ by selecting the highest values
    \State $\textbf{D}$ = \textbf{SearchForTopkDocuments}($q', I^1, k$) // i.e SPLADE, SPLADE-BM25...
    \State Initialize dictionary \textit{scores}
    \For{$d_{id}$ in $\textbf{D}$}
        \State $d$ = $I^2_{d_{id}}$ // Recover the unpruned document representation
        \State $score$ = dot($d$,$q$) // Compute the unpruned query and document score
        \State $scores$[$d_{id}$] = score // Store it
    \EndFor
    \State \textbf{Return} scores
\end{algorithmic}
\end{algorithm}


Actually, there are already many ``first-stage'' systems that implement a similar system. For example, the classical \textbf{I}n\textbf{V}erted \textbf{F}ile index (IVF) works by similarly splitting the ``first-stage'' of retrieval into two parts. First, it limits the search over the cluster centroids and it selects a number of clusters to explore, then it properly scores the documents. Another system that works similarly in two steps is \textbf{P}roduct \textbf{Q}uantization (PQ): distances are computed with quantized vectors first and then residuals are applied to improve the approximation of the true distance. In summary, we are the first to propose this in the context of ``learned sparse representation''\footnote{as far as we are aware...}, even if the idea itself is not completely novel.

\section{Experiments}

\subsection{Implementation}

We set up our experiments on the Anserini codebase. We take advantage of the new ONNX module on Anserini and all the optimizations it brings (including int8 quantization) in order to reduce query encoding times. All these integrations allow us, for the first time, to actually have a full end-to-end system in a single ''language``/''framework``, instead of taking measurements separately. Also, this means that we can properly compare the costs of BM25 and SPLADE in a latency sense, with the only caveat being the increased index size (see Section~\ref{sec:index size}).


\subsection{In-domain experiments}

For MSMARCO-v1 we use the 6980 queries dev set and present results in Figure~\ref{fig:integrated_v1}. Models are able to achieve 38.20 MRR@10 in 21 ms on Anserini considering all steps (for comparison, DocT5 takes 28 ms for 27.23 MRR@10). Just reranking the top100 of DocT5 is quite effective, but the whole SPLADE process (encoding + reranking) takes around 20ms making it less efficient than just using a less accurate SPLADE in the first pass.

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v1_new.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over MSMARCO v1 devset on Anserini with all steps considered.}
    \label{fig:integrated_v1}
\end{figure}

For MSMARCO-v2 we use the 76 queries TREC-DL 2022 set, which could be too small, but the MSMARCO-v2 devsets are not recommended. Results are presented in Figure~\ref{fig:integrated_v2}. We note that the models are able to scale to 130M, achieving 0.56 nDCG@10 (SPLADE++ achieves 0.57 and takes so long it would break the Figure) in 82 ms (which is faster than BM25 on MSMARCO v2 and even our Efficient models on MSMARCO v1).

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v2_new.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over TREC-DL-2022 on Anserini with all steps considered.}
    \label{fig:integrated_v2}
\end{figure}

The "secret" ingredient is the use of BM25 scoring (i.e. use SPLADE weights as TF with BM25) instead of IMPACT/SPLADE. It greatly improves efficiency, but reduces drastically effectiveness (that can be recovered later on the second stage). Further investigation is needed, but the impact is much more apparent on MSMARCO v2.

\subsection{Index size}
\label{sec:index size}

For all these experiments everything has been preloaded to memory to try to avoid getting inconsistent results via cache and for improving the overall speed, but it can be quite hefty for MSMARCO v2. Table~\ref{tab:sizes} presents the index sizes, showing that reranking MSMARCO v1 can take up to 4.5Gb, but v2 takes up to 85Gb. This could be reduced by not keeping the ``second-stage'' index in memory, but I would need to redo all experiments for that.

\begin{table}[ht]
\begin{center}
\caption{Index sizes in megabytes.}
\label{tab:sizes}
\begin{tabular}{c|cc}
\toprule
Model              & MSMARCO v1 & MSMARCO v2 \\
\midrule
\multicolumn{3}{c}{First Stage Only}         \\
\midrule
BM25               & 509        & 10140      \\
DOCT5              & 855        & 16905      \\
Pruned 32   SPLADE & 760        & 13813      \\
SPLADE             & 3680       & 66349      \\
\midrule
\multicolumn{3}{c}{First+Second Stage}                   \\
\midrule
BM25               & 4189       & 76489      \\
DOCT5              & 4535       & 83254      \\
Pruned 32   SPLADE & 4440       & 80162     \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}

However, many previous works advise against using segments larger than 10M documents, so it should not be that much of a problem if we can stay in the 4.5Gb range per segment/machine. Not sure if we want to delve into this, but could be pretty interesting and have a direct connection to elastic search (who manages automatically the segments)

==> draft.tex <==
\section{Introduction}

Given our recent results and other articles in the literature, the most significant way to improve the latency of SPLADE models has been to reduce the number of query terms, followed by some distance by the pruning of document terms. However, when we approach very fast models ($\approx$ BM25 latency) we start noticing a sharp drop in effectiveness, especially in out-of-domain experiments. 

One way to counter-act this is to limit the number of documents searched with the expanded terms. We propose to use a two-stage retrieval: i) in the first stage we use only non expanded terms and retrieve a top-$k$; and ii) rerank the top-$k$ using the full documents and queries from SPLADE. In the following we call Lexical-SPLADE (L) the approach where we remove all expansion and QLexical-SPLADE (QL) the one that we remove expansion only from the query.

\section{Experiments}

\subsection{Validating approach}

For the first set of experiments, we consider that reranking is free. While this is not true, the idea is to validate the effectiveness of reranking and the efficiency gains from changing the first stage. We use three SPLADE models: i) Efficient SPLADE-V-Large (Eff-V-L) ii) SPLADE++ ensemble distil (ed); iii) SPLADE++ self distil (sd); and iv) Further distillation over sd (best). Results are presented in Figure~\ref{fig:without_rerank_msmarco} (MSMARCO) and Figure~\ref{without_rerank_beir} (BEIR). We validate the approach as the first stage is much faster than full retrieval and reranking is able to recover almost all the effectiveness of the original model. It is also the first time that we are able to improve latency and not lose effectiveness on BEIR. Note that reranking is always done over the top1k documents.

\input{tikz/without_reranking/MSMARCO/figure}

\input{tikz/without_reranking/BEIR/figure}

\subsection{First reranking implementation}

We now test a first implementation of the reranking. The idea is to give us an upper bound of the cost of reranking and it can be improved. We consider that PISA sends us a list of top-$k$ documents, but no representation, meaning that we need to add two things: i) Document loading and ii) proper reranking. Implementation is done in pure python and we run over the "BEST" model, with the Lexical-SPLADE as the first stage. Results are displayed in Figure~\ref{with_rerank_msmarco}, showing that with a good implementation of ``document loading'' the two stage SPLADE works pretty well.

\input{tikz/with_reranking/MSMARCO/figure}

\input{tikz/with_reranking/MSMARCO/figure2}

For document loading, we first store all documents as separate files, with documents represented as a dictionary encoded in JSON. This is very inefficient and costly (around 30 GBs of space). In the case that we only remove items from the query (QL) it is simple to see how the system itself could perform this step and send it to the reranker, but in the case of a simplified version (L) it is harder to see. I've one current implementation of this where it takes around 0.1 ms per document, with $k=100$ taking 12 ms, $k=250$ taking 22ms and $k=1000$ taking 124 ms.

For reranking I'm currently using a brute force approach with a per-query complexity of $O(k*q)$ where $k$ is the amount of documents to rerank and q is the amount of query terms. This step is way faster than document loading, with $k=100$ taking $0.3$ ms per query, $k=250$ taking $0.8$ ms per query and $k=1000$ taking $3.9$ ms per query.

\subsection{Comparing with pruning}

In the previous experiments we were only considering lexically pruning the document index. We could also prune with document-centric pruning as in our previous work. We now add SPLADE with document pruning (D-SPLADE) and its combination with lexical query pruning (DLQ-SPLADE). 

\input{tikz/with_reranking/MSMARCO_pruning/figure}

\newpage

\subsection{Integrating everything}

Now we go back to Anserini in order to be able to integrate all steps into the same software. We integrate query inference (using onnx and int8 quantization) and the two-stage SPLADE in a single run. This means that barring the extra costs of the larger SPLADE index (and its smaller thresholded version), both BM25 and SPLADE are evaluated with the same cost.

Considering the results from the previous experiments we now will consider only document-centric pruning (top k = 4,8,16,32,64) and query-centric pruning (top k=5). Reranking is done on the top 100.

For MSMARCO-v1 we use the 6980 queries dev set and present results in Figure~\ref{fig:integrated_v1}. Models are able to achieve 38.20 MRR@10 in 21 ms on Anserini considering all steps (for comparison, DocT5 takes 28 ms for 27.23 MRR@10). Just reranking the top100 of DocT5 is quite effective, but the whole SPLADE process (encoding + reranking) takes around 20ms making it less efficient than just using a less accurate SPLADE in the first pass.

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v1-filtered.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over MSMARCO v1 devset on Anserini with all steps considered.}
    \label{fig:integrated_v1}
\end{figure}

For MSMARCO-v2 we use the 76 queries TREC-DL 2022 set, which could be too small, but the MSMARCO-v2 devsets are not recommended. Results are presented in Figure~\ref{fig:integrated_v2}. We note that the models are able to scale to 130M, achieving 0.56 nDCG@10 (SPLADE++ achieves 0.57 and this model 0.62) in 82 ms (which is faster than BM25 on MSMARCO v2 and even our Efficient models on MSMARCO v1).

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v2-filtered.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over TREC-DL-2022 on Anserini with all steps considered.}
    \label{fig:integrated_v2}
\end{figure}

The "secret" ingredient is the use of BM25 scoring (i.e. use SPLADE weights as TF with BM25) instead of IMPACT/SPLADE. It greatly improves efficiency, but reduces drastically effectiveness (that can be recovered later on the second stage). I'm not 100\% sure why this happens (probably acting as a secondary pruning by term weights?), but the impact is much more apparent on MSMARCO v2.

Finally, one thing to note is that for now, these are quite memory intensive. For all these experiments everything has been preloaded to memory to try to avoid getting inconsistent results via cache and for improving the overall speed, but it can be quite hefty for MSMARCO v2. Table~\ref{tab:sizes} presents the index sizes, showing that reranking MSMARCO v1 can take up to 4.5Gb, but v2 takes up to 85Gb. This could be reduced by not keeping the reranker index in memory, but I would need to redo all experiments for that (so for a next iteration).

\begin{table}[ht]
\caption{Index sizes in megabytes.}
\label{tab:sizes}
\begin{tabular}{c|cc}
\toprule
Model              & MSMARCO v1 & MSMARCO v2 \\
\midrule
\multicolumn{3}{c}{First Stage Only}         \\
\midrule
BM25               & 509        & 10140      \\
DOCT5              & 855        & 16905      \\
Pruned 32   SPLADE & 760        & 13813      \\
SPLADE             & 3680       & 66349      \\
\midrule
\multicolumn{3}{c}{Rerank}                   \\
\midrule
BM25               & 4189       & 76489      \\
DOCT5              & 4535       & 83254      \\
Pruned 32   SPLADE & 4440       & 80162     \\ 
\bottomrule
\end{tabular}
\end{table}

However, many previous works don't advise using segments larger than 10M documents, so it should not be that much of a problem if we can stay in the 4.5Gb range per segment/machine. Not sure if we want to delve into this, but could be interesting.

\subsection{Full images}

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v1-bm25.pdf}
        }
    \end{subfigure}
    \caption{Two stage BM25 with different methods on V1.}
    \label{fig:integrated_v2t5}
\end{figure}


\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v2-filtered.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over TREC-DL-2022 on Anserini with all steps considered over top500.}
    \label{fig:integrated_v2t5}
\end{figure}


\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v1.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over MSMARCO v1 devset on Anserini with all steps considered.}
    \label{fig:integrated_v1f}
\end{figure}


\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v2.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over TREC-DL-2022 on Anserini with all steps considered.}
    \label{fig:integrated_v2f}
\end{figure}


\section{Other things we can test}

There is probably something in the sense of PRF that we can do if we are separating in two steps$\dots$

==> figures/tmp.tex <==


%\subsection{PRF/Reranking}
%Pseudo relevance feedback (PRF) is the idea of using the retrieved set of documents to augment the query and improve results. Considering all the pruning that was already done, we ask the question of what would happen if instead of using the tokens present in the pruned version of documents we did a PRF where the feedback comes from the unprunned documents and queries.


==> id.tex <==
\section{Introduction}

Given our recent results and other articles in the literature, the most significant way to improve the latency of SPLADE models has been to reduce the number of query terms, followed by some distance by the pruning of document terms. However, when we approach very fast models ($\approx$ BM25 latency) we start noticing a sharp drop in effectiveness, especially in out-of-domain experiments. We provide empirical evidence in Table~\ref{tab:summary}.

\input{tables/summary.tex}

One way to counter-act this is to limit the number of documents searched with the expanded query terms. To do so, we split our first-stage ranking into two steps: i) in the first stage we prune aggressively so that both queries and documents have statistics similar to a non expanded dataset\footnote{For example, on MSMARCO we limit ourselves to 5 tokens per query and 32 per document} and return a top-$k$; and ii) rerank the top-$k$ using the full documents and queries from SPLADE. For now we always consider the same SPLADE model for both steps, but this could be improved by using two different models (although with increased latency due to paying the query encoding twice).

\section{Method}

In order to achieve the best of both worlds: i) Fast retrieval; and ii) Accurate out-of-domain effectiveness, we aim to combine our methods. The main goal is that for most documents we perform very simple and fast computations (See IDs 1 and 2 which describe exactly how to get those faster SPLADE implementations) and then after getting a small set of candidates (around 100) we allow the system to perform slightly more costly computation. This is indeed how most systems are implemented, with a ``first-stage`` and ''second-stage`` retrieval, where most of the time the first-stage is a vector-based retrieval and the second stage a cross-encoder. While SPLADE mostly belongs to the first-stage, there's nothing that obliges it to perform retrieval in a single step. So we actually propose to split the retrieval, with the first stage being a very rough representation of the representations (aggressive document and query pruning) and the second stage using the actual representation.\footnote{Maybe we could imagine a residual system later?} We describe this algorithm in Algorithm~\ref{alg:pruning} (Preprocessing) and Algorithm~\ref{alg:query} (Two stage processing).

\begin{algorithm}
\caption{Preprocessing: Pruning models}\label{alg:pruning}
\begin{algorithmic}[1]
\Require{$T$ collection, $Q$ collection, preprocessed for SPLADE}
\State Compute averages of $T$ and $Q$ and store as $l_d$ and $l_q$
\State \textbf{Initialize} $I^1$ as an empty index // Pruned document index
\State \textbf{Initialize} $I^2$ as an empty index // Full document index
\For{each document $d$ in $T$}
    \State $d' = $Prune $d$ to size $l_d$ by selecting the highest values
    \State Add $d'$ to $I^1$
    \State Add $d$ to $I^2$
    
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Two stage Processing Algorithm}\label{alg:query}
\begin{algorithmic}[1]
\Require{Indexes $I^1$ and $I^2$, a query $q$, an average query size $l_q$ and the amount of documents to return $k$}
    \State $q' = $Prune $q$ to size $l_q$ by selecting the highest values
    \State $\textbf{D}$ = \textbf{SearchForTopkDocuments}($q', I^1, k$) // i.e SPLADE, SPLADE-BM25...
    \State Initialize dictionary \textit{scores}
    \For{$d_{id}$ in $\textbf{D}$}
        \State $d$ = $I^2_{d_{id}}$ // Recover the unpruned document representation
        \State $score$ = dot($d$,$q$) // Compute the unpruned query and document score
        \State $scores$[$d_{id}$] = score // Store it
    \EndFor
    \State \textbf{Return} scores
\end{algorithmic}
\end{algorithm}


Actually, there are already many ``first-stage'' systems that implement a similar system. For example, the classical \textbf{I}n\textbf{V}erted \textbf{F}ile index (IVF) works by similarly splitting the ``first-stage'' of retrieval into two parts. First, it limits the search over the cluster centroids and it selects a number of clusters to explore, then it properly scores the documents. Another system that works similarly in two steps is \textbf{P}roduct \textbf{Q}uantization (PQ): distances are computed with quantized vectors first and then residuals are applied to improve the approximation of the true distance. In summary, we are the first to propose this in the context of ``learned sparse representation''\footnote{as far as we are aware...}, even if the idea itself is not completely novel.

\section{Interest for Naver}

Improving the efficiency of SPLADE methods is important for its use in practice, even if it comes with the cost of slightly changing the implementation on the systems (as it needs to run as a pipeline instead of a single call).

\section{Experiments}

\subsection{Implementation}

We set up our experiments on the Anserini codebase. We take advantage of the new ONNX module on Anserini and all the optimizations it brings (including int8 quantization) in order to reduce query encoding times. All these integrations allow us, for the first time, to actually have a full end-to-end system in a single ''language``/''framework``, instead of taking measurements separately. Also, this means that we can properly compare the costs of BM25 and SPLADE in a latency sense, with the only caveat being the increased index size (see Section~\ref{sec:index size}).


\subsection{In-domain experiments}

For MSMARCO-v1 we use the 6980 queries dev set and present results in Figure~\ref{fig:integrated_v1}. Models are able to achieve 38.20 MRR@10 in 21 ms on Anserini considering all steps (for comparison, DocT5 takes 28 ms for 27.23 MRR@10). Just reranking the top100 of DocT5 is quite effective, but the whole SPLADE process (encoding + reranking) takes around 20ms making it less efficient than just using a less accurate SPLADE in the first pass.

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v1_new.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over MSMARCO v1 devset on Anserini with all steps considered.}
    \label{fig:integrated_v1}
\end{figure}

For MSMARCO-v2 we use the 76 queries TREC-DL 2022 set, which could be too small, but the MSMARCO-v2 devsets are not recommended. Results are presented in Figure~\ref{fig:integrated_v2}. We note that the models are able to scale to 130M, achieving 0.56 nDCG@10 (SPLADE++ achieves 0.57 and takes so long it would break the Figure) in 82 ms (which is faster than BM25 on MSMARCO v2 and even our Efficient models on MSMARCO v1).

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\textwidth}
        \centering
        \adjustbox{max width=\textwidth}{%
            \includegraphics{figures/MSMARCO-v2_new.pdf}
        }
    \end{subfigure}
    \caption{Two stage SPLADE over TREC-DL-2022 on Anserini with all steps considered.}
    \label{fig:integrated_v2}
\end{figure}

The "secret" ingredient is the use of BM25 scoring (i.e. use SPLADE weights as TF with BM25) instead of IMPACT/SPLADE. It greatly improves efficiency, but reduces drastically effectiveness (that can be recovered later on the second stage). Further investigation is needed, but the impact is much more apparent on MSMARCO v2.

\subsection{Index size}
\label{sec:index size}

For all these experiments everything has been preloaded to memory to try to avoid getting inconsistent results via cache and for improving the overall speed, but it can be quite hefty for MSMARCO v2. Table~\ref{tab:sizes} presents the index sizes, showing that reranking MSMARCO v1 can take up to 4.5Gb, but v2 takes up to 85Gb. This could be reduced by not keeping the ``second-stage'' index in memory, but I would need to redo all experiments for that.

\begin{table}[ht]
\begin{center}
\caption{Index sizes in megabytes.}
\label{tab:sizes}
\begin{tabular}{c|cc}
\toprule
Model              & MSMARCO v1 & MSMARCO v2 \\
\midrule
\multicolumn{3}{c}{First Stage Only}         \\
\midrule
BM25               & 509        & 10140      \\
DOCT5              & 855        & 16905      \\
Pruned 32   SPLADE & 760        & 13813      \\
SPLADE             & 3680       & 66349      \\
\midrule
\multicolumn{3}{c}{First+Second Stage}                   \\
\midrule
BM25               & 4189       & 76489      \\
DOCT5              & 4535       & 83254      \\
Pruned 32   SPLADE & 4440       & 80162     \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}

However, many previous works advise against using segments larger than 10M documents, so it should not be that much of a problem if we can stay in the 4.5Gb range per segment/machine. Not sure if we want to delve into this, but could be pretty interesting and have a direct connection to elastic search (who manages automatically the segments)

==> preamble_acm.tex <==
%%
%% This is file `sample-manuscript.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% samples.dtx  (with options: `manuscript')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from sample-manuscript.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file samples.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Commands for TeXCount
%TC:macro \cite [option:text,text]
%TC:macro \citep [option:text,text]
%TC:macro \citet [option:text,text]
%TC:envir table 0 1
%TC:envir table* 0 1
%TC:envir tabular [ignore] word
%TC:envir displaymath 0 word
%TC:envir math 0 word
%TC:envir comment 0 0
%%
%%
%% The first command in your LaTeX source must be the \documentclass command.
%%%% Small single column format, used for CIE, CSUR, DTRAP, JACM, JDIQ, JEA, JERIC, JETC, PACMCGIT, TAAS, TACCESS, TACO, TALG, TALLIP (formerly TALIP), TCPS, TDSCI, TEAC, TECS, TELO, THRI, TIIS, TIOT, TISSEC, TIST, TKDD, TMIS, TOCE, TOCHI, TOCL, TOCS, TOCT, TODAES, TODS, TOIS, TOIT, TOMACS, TOMM (formerly TOMCCAP), TOMPECS, TOMS, TOPC, TOPLAS, TOPS, TOS, TOSEM, TOSN, TQC, TRETS, TSAS, TSC, TSLP, TWEB.
% \documentclass[acmsmall]{acmart}

%%%% Large single column format, used for IMWUT, JOCCH, PACMPL, POMACS, TAP, PACMHCI
% \documentclass[acmlarge,screen]{acmart}

%%%% Large double column format, used for TOG
% \documentclass[acmtog, authorversion]{acmart}

%%%% Generic manuscript mode, required for submission
%%%% and peer review
\usepackage{enumitem}[nolistsep]
\usepackage{multirow} 
\usepackage{array}
\usepackage[para]{footmisc}
\usepackage{bbm}
\usepackage{adjustbox}
\usepackage{pgfplots}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{pgfkeys}
\usepackage[normalem]{ulem}
%\useunder{\uline}{\ul}{}

\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}


\usepackage[show]{chato-notes}

%\newcommand{\nic}[1]{\textcolor{blue}{#1}} 
\newcommand{\nic}[1]{{#1}} %blue
%\newcommand{\car}[1]{\textcolor{red}{#1}} %blue
\newcommand{\car}[1]{{#1}} %blue

%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}

%\copyrightyear{2023}
%\acmYear{2023}
%\setcopyright{acmlicensed}\acmConference[SIGIR '23]{Proceedings of the 46th
%International ACM SIGIR Conference on Research and Development in
%Information Retrieval}{July 23--27, 2023}{Taipei, Taiwan}
%\acmBooktitle{Proceedings of the 46th International ACM SIGIR Conference on
%Research and Development in Information Retrieval (SIGIR '23), July 23--27,
%2023, Taipei, Taiwan}
%\acmPrice{15.00}
%\acmDOI{10.1145/3539618.3591941}
%\acmISBN{978-1-4503-9408-6/23/07}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% For managing citations, it is recommended to use bibliography
%% files in BibTeX format.
%%
%% You can then either use BibTeX with the ACM-Reference-Format style,
%% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
%% support for advanced citation of software artefact from the
%% biblatex-software package, also separately available on CTAN.
%%
%% Look at the sample-*-biblatex.tex files for templates showcasing
%% the biblatex styles.
%%

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

%%
%% end of the preamble, start of the body of the document source.


==> tables/per_beir.tex <==
\begin{table}[]
\caption{Per dataset latencies - BEIR}
\label{tab:lat-per-beir}
\adjustbox{max width=1.0\columnwidth}{%
\begin{tabular}{@{}c|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{dataset} & \multicolumn{2}{c}{avg\_latency} & \multicolumn{2}{c}{med\_latency} & \multicolumn{2}{c}{q99\_latency} \\ \cmidrule(l){2-7} 
                 & BM25      & OURS (row g) & BM25  & OURS (row g) & BM25   & OURS (row g) \\ \midrule
arguana            & 2.0  & 1.8  & 1.8 & 1.8  & 4.9  & \textbf{2.6}  \\
bioasq             & 10.0 & 28.4 & 6.4 & 26.4 & 50.9 & 67.1 \\
climate-fever      & 13.1 & 6.8  & 9.7 & 6.2  & 59.0 & \textbf{16.9} \\
dbpedia-entity     & 3.0  & 2.7  & 1.8 & 2.5  & 15.8 & \textbf{5.7}  \\
fever              & 3.2  & 4.8  & 2.2 & 4.6  & 14.8 & \textbf{11.6} \\
fiqa               & 0.7  & 1.3  & 0.6 & 1.3  & 2.1  & 2.5  \\
hotpotqa           & 8.1  & 6.5  & 6.6 & 5.9  & 29.3 & \textbf{17.0} \\
nfcorpus           & 0.0  & 0.3  & 0.0 & 0.3  & 0.2  & 0.5  \\
nq                 & 3.5  & 2.3  & 3.0 & 2.1  & 10.6 & \textbf{5.3}  \\
quora              & 0.5  & 0.6  & 0.4 & 0.6  & 2.1  & \textbf{1.4}  \\
robust04           & 4.3  & 3.9  & 2.9 & 3.7  & 24.2 & \textbf{8.1}  \\
scidocs            & 0.3  & 0.9  & 0.3 & 0.8  & 0.8  & 2.1  \\
scifact            & 0.2  & 1.4  & 0.2 & 1.5  & 0.4  & 2.3  \\
signal1m           & 1.9  & 3.4  & 1.7 & 3.5  & 6.3  & 7.0  \\
trec-covid         & 1.5  & 3.3  & 1.3 & 3.2  & 5.2  & 5.7  \\
trec-news          & 3.4  & 4.0  & 3.1 & 3.9  & 10.9 & \textbf{6.8}  \\
webis-touche2020   & 1.0  & 1.7  & 0.9 & 1.5  & 2.6  & 4.0  \\ \midrule
Faster           & 9         & 8            & 13    & 4            & 8      & 9            \\
Average (not ideal)       & 3.3     & 4.3     & 2.5     & 4.1     & 14.1     & 9.8     \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/per_beir_2.tex <==
\begin{table}[]
\caption{Per dataset latencies - BEIR - Against UCSB works}
\label{tab:lat-per-beir}
\adjustbox{max width=1.0\columnwidth}{%
\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
\multirow{2}{*}{dataset} & \multicolumn{3}{c}{avg\_latency} & \multicolumn{3}{c}{nDCG@10}  \\ \cmidrule(l){2-7} 
                         & 2GTI/s-fast~\cite{qiao2023optimizing} & HT3~\cite{qiao2023representation} & OURS (row g) & 2GTI/s-fast~\cite{qiao2023optimizing} & HT3~\cite{qiao2023representation} & OURS (row g) \\ \midrule

arguana            & 8.8   & 4.1   & \textbf{1.8} & 44.8 & \textit{50.0} & \textit{50.0} \\
climate-fever      & 355.0 & 332.0 & \textbf{6.8} & \textbf{23.1} & 21.3 & 22.1 \\
dbpedia-entity     & 34.5  & 32.3  & \textbf{2.7} & \textbf{44.9} & 42.6 & 43.8 \\
fever              & 655.0 & 264.0 & \textbf{4.8} & \textbf{77.1} & 76.4 & 77.0 \\
fiqa               & 3.4   & 3.2   & \textbf{1.3} & 35.4 & 33.6 & \textbf{37.3} \\
hotpotqa           & 191.0 & 140.0 & \textbf{6.5} & \textbf{68.1} & 67.8 & 67.3 \\
nfcorpus           & \textit{0.2}   & \textit{0.2}  & 0.3 & 34.7 & 34.6 & \textbf{35.4} \\
nq                 & 28.6  & 28.6  & \textbf{2.3} & 55.1 & 53.9 & \textbf{57.4} \\
quora              & 21.5  & 9.2   & \textbf{0.6} & \textit{81.7} & 79.2 & \textit{81.7} \\
scidocs            & 2.1   & 3.0   & \textbf{0.9} & 15.5 & 15.1 & \textbf{15.8} \\
scifact            & 2.9   & \textit{1.4}   & \textit{1.4} & 68.0 & 67.2 & \textbf{71.1} \\
trec-covid         & 9.9   & 7.5   & \textbf{3.3} & 70.7 & 69.5 & \textbf{74.0} \\
webis-touche2020   & 3.2   & 4.5   & \textbf{1.7} & 29.1 & \textbf{31.3} & 29.7 \\ \midrule
Better             & 0.5   & 1.0   & 11.5  & 4.5  & 1.5  & 7.0  \\
Average (not ideal) & 101.2 & 63.8  & \textbf{2.6} & 49.9 & 49.4 & \textbf{51.0}

                         
\end{tabular}
}
\end{table}


==> tables/per_lotte.tex <==
\begin{table}[]
\caption{Per dataset latencies - Lotte}
\label{tab:per-lotte}
\adjustbox{max width=1.0\columnwidth}{%
\begin{tabular}{@{}c|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{dataset} & \multicolumn{2}{c}{avg\_latency} & \multicolumn{2}{c}{med\_latency} & \multicolumn{2}{c}{q99\_latency} \\ \cmidrule(l){2-7}
                         & BM25        & OURS (row g)       & BM25        & OURS (row g)       & BM25        & OURS (row g)       \\ \midrule
forum-lifestyle    & 0.6 & 1.3 & 0.5 & 1.2 & 2.4  & 3.1  \\
forum-recreation   & 0.6 & 1.1 & 0.5 & 1.0 & 2.3  & 2.3  \\
forum-science      & 3.2 & 7.3 & 2.4 & 5.8 & 12.6 & 25.1 \\
forum-technology   & 1.7 & 4.5 & 1.4 & 4.0 & 5.9  & 12.0 \\
forum-writing      & 0.8 & 1.2 & 0.6 & 1.1 & 4.1  & \textbf{2.8}  \\
search-lifestyle   & 0.5 & 1.2 & 0.4 & 1.1 & 2.1  & 2.8  \\
search-recreation  & 0.6 & 1.6 & 0.5 & 1.4 & 2.1  & 3.4  \\
search-science     & 2.9 & 2.8 & 2.2 & 2.0 & 12.3 & \textbf{12.2} \\
search-technology  & 1.7 & 2.5 & 1.3 & 2.3 & 6.2  & 6.6  \\
search-writing     & 0.9 & 1.4 & 0.7 & 1.3 & 3.6  & \textbf{3.3}  \\ \midrule
Faster             & 9   & 1   & 9   & 1   & 7    & 3    \\
Average (not ideal) & 1.4 & 2.5 & 1.0 & 2.1 & 5.4  & 7.3  \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/reranking.tex <==
\begin{table}[ht]
\caption{Reranking eff-V-SPLADE-L with static pruning. Latency considers only the first stage step. $^\dagger$ indicates statistical significant drop compared to the reranked baseline.}
\label{tab:reranking}
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Max size}  & \multicolumn{2}{c}{MSMARCO dev}      & \multicolumn{2}{c}{TREC-DL 2019} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& Latency ($\times$)     & MRR@10 & Latency ($\times$)     & nDCG@10    \\
\midrule
\multicolumn{5}{c}{Baseline without reranking} \\
\midrule
\car{30 522}     & 28.0 (1.0$\times$)           & 38.9\hphantom{$^\dagger$} & 28.2 (1.0$\times$)           & 71.4 \\
\midrule
\multicolumn{5}{c}{Baseline with reranking} \\
\midrule
\car{30 522}     & 28.0 (1.0$\times$)          & 42.8\hphantom{$^\dagger$} & 28.2 (1.0$\times$)           & 77.1 \\
\midrule
\multicolumn{5}{c}{Prune by document size (D)} \\
\midrule
%128       & 10.69 (1.01x) & 42.6 & 42.8 & 11.33 (0.99x) & 42.6 & 42.8 \\
64        & 13.0 (2.2$\times$) & 42.9\hphantom{$^\dagger$} & 14.1 (2.1$\times$) & 77.0 \\
32        & 7.1 (4.0$\times$) & 42.7\hphantom{$^\dagger$} & 10.3 (3.2$\times$) & 75.8 \\
16        & 3.7 (7.6$\times$) & 42.4$^\dagger$ & 8.4 (4.7$\times$) & 76.4 \\
8         & 2.0 (13.9$\times$) & 41.5$^\dagger$ & 5.9 (6.4$\times$) & 75.6 \\
4         & 1.0 (27.0$\times$) & 38.8$^\dagger$ & 3.4 (16.6$\times$) & 74.1 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/reranking_new.tex <==
\begin{table}[ht]
\caption{Effectiveness effect size analysis ($p\leq 0.01$) of reranking using 3 different models against the two-stage SPLADE (row g on main table).}
\label{tab:reranking}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{Comparison   against Two Stage SPLADE (+ means improve over TwoStageSPLADE)} \\ \midrule
                                                  & Summary Effect     & +      & =     & -     \\ \midrule
BM25 -\textgreater MiniLM Top100                  & -0,04            & 15     & 13    & 14    \\ \midrule
BM25 -\textgreater DeBERTA Top10                  & -3,53            & 7      & 15    & 20    \\
BM25 -\textgreater DeBERTA Top50                  & 2,92             & 31     & 4     & 7     \\ \midrule
TwoStage SPLADE -\textgreater Deberta   Top10     & 2,94             & 36     & 5     & 1     \\ 
TwoStage SPLADE -\textgreater Deberta   Top50     & 5,97             & 38     & 3     & 1     \\ \bottomrule
\end{tabular}
\end{table}


==> tables/summary.tex <==
\begin{table}[h!]
\caption{Result summary. Latency numbers are averaged over all queries and do not contain encoding times. Bold is best in column, italic second best and underline third best. Change scoring means using BM25 scoring over SPLADE weights for the first stage instead of using impact (i.e. dot product).}
\label{tab:summary}

\adjustbox{max width=\columnwidth}{%
\begin{tabular}{c|cccc|ccc}
\toprule
\multirow{2}{*}{Model}                                                    & \multicolumn{4}{c}{MSMARCO v1}                                & \multicolumn{3}{c}{BEIR}                                                                 \\
                                                                          & Latency       & Dev           & TREC19        & TREC20        & 13 nDCG@10 & \textgreater{}1M nDCG@10 & \textgreater{}1M latency \\ \midrule
\multicolumn{8}{c}{Baselines}                                                                                                                                                                                                        \\ \midrule
BM25 without stopwords                                                    & \textit{22}   & 18,8          & 50,6          & 48,8          & 44,9               & 44,2                             & N/A                              \\
Splade PPSD                                                               & $\approx$2400          & 37,8          & \textbf{72,7} & 72,1          & \underline{50,6}         & \underline{53,7}                       & N/A                              \\
Efficient V                                                               & 300           & 38,8          & 71,3          & 71,4          & 47,7               & 51,3                             & N/A                              \\ \midrule
\multicolumn{8}{c}{Latest developments}                                                                                                                                                                                                          \\ \midrule
a) New SPLADE (base)                                                & 885           & \textbf{40,2} & \underline{72,2}    & \textbf{75,2} & \textbf{51,6}      & \textbf{54,9}                    & N/A                              \\
b) +Pruning (a+b)                                                & \underline{30}      & 36,3          & 68,9          & 67,6          & 45,7               & 46,1                             & \textit{31}                      \\
\midrule
\multicolumn{8}{c}{This ID}                                                                                                                                                                                                          \\ \midrule
c) +RerankTop100 (a+b+c)                                       & 38            & \textit{39,9} & 71,9          & \underline{74,7}    & \textit{51,1}      & \textit{54,0}                    & \underline{46}                         \\
d) +Change Scoring (a+b+c+d) & \textbf{12} & \underline{39,6}    & \textit{72,4} & \textit{74,9} & 50,0               & 51,4                             & \textbf{29}     \\ \bottomrule                
\end{tabular}
}
\end{table}


==> tables/summary_ppsd.tex <==
\begin{table}[ht]
\centering
\caption{Effectiveness effect size analysis ($p\leq 0.01$) of methods PPSD SPLADE (b) and Pseudo-Guided Traversal (PGT). Latency is normalized by BM25 (1.0 is equal to BM25) and are the lower the better. >1M means the subset of datasets of BEIR that have at least 1M documents on the corpus (i.e. excluding small datasets where measuring latency is less relevant).}
\label{tab:summary_ppsd}

\adjustbox{max width=0.95\columnwidth}{%
\begin{tabular}{@{}c|c|cccc|cccc|cc|cc|c@{}}
\toprule
\multirow{3}{*}{\#} & \multirow{3}{*}{Method} & \multicolumn{8}{c|}{Effect   size against}             & \multicolumn{2}{c|}{MSMARCO}                        & \multicolumn{2}{c|}{BEIR} & \multirow{2}{*}{Lotte} \\ \cmidrule(l){3-14} 
                  &                         & \multicolumn{4}{c|}{PGT (d)} & \multicolumn{4}{c|}{SPLADE (b)} & \multicolumn{2}{c|}{Latency} & 18    & \textgreater{}1M &       \\
                  &                         & Mean   & +    & =   & -  & Mean   & +   & =    & -    & Average   & p99                      & \multicolumn{2}{c|}{AvG L}              & AvG L         \\ \midrule
\multicolumn{15}{c}{Baselines}   \\
\midrule 
a & BM25   & -8.9 & 1  & 4  & 25 & -10.2 & 1 & 5 & 24 & 1.0  & 1.0  & 1.0  & 1.0  & 1.0  \\
b & PPSD SPLADE & 1.3  & 15 & 12 & 3  & \multicolumn{4}{c|}{N/A}  & 68.9 & 41.0 & 57.7 & 70.5 & 41.7 \\
\midrule 
\multicolumn{15}{c}{Advanced Baselines}   \\ \midrule 
c & (b) pruned to dataset original statistics      & -3.0 & 0 & 14 & 16       & -4.3 & 0 & 5  & 25 & 0.7 & 0.4 & 2.9 & 3.2 & 2.6 \\
d & \textbf{P}seudo-\textbf{G}uided \textbf{T}raversal ($a \xrightarrow{} b$) & \multicolumn{4}{c|}{N/A} & -0.7 & 3 & 12 & 15 & 1.3 & 1.1 & 1.4 & 1.3 & 1.6 \\
\midrule 
\multicolumn{15}{c}{This work}   \\
\midrule 
e & Re-weighted documents of (c) with $k1=100$           & -5.2 & 0  & 5  & 25 & -6.5 & 0 & 4  & 26 & 0.6 & 0.4 & 1.5 & 1.7 & 1.6 \\
f & Two-Step ($c \xrightarrow{} b$)      & 1.0  & 15 & 10 & 5  & -0.2 & 0 & 20 & 10 & 1.0 & 0.5 & 3.0 & 3.2 & 3.1 \\
g & Two-Step ($e \xrightarrow{} b$) & 0.8  & 15 & 10 & 5  & -0.5 & 0 & 17 & 13 & 0.8 & 0.4 & 1.8 & 1.9 & 2.0 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/summary_summarized.tex <==
\begin{table}[ht]
\centering
\caption{Effectiveness effect size analysis ($p\leq 0.01$) of methods SPLADE (b) and Pseudo-Guided Traversal (PGT). Latency is normalized by BM25 (1.0 is equal to BM25) and are the lower the better. >1M means the subset of datasets of BEIR that have at least 1M documents on the corpus (i.e. excluding small datasets where measuring latency is less relevant).}
\label{tab:summary_old}

\adjustbox{max width=1.0\columnwidth}{%
\begin{tabular}{@{}cc|cccc|cccc|cc|cc|c@{}}
\toprule
\multirow{3}{*}{\#} & \multirow{3}{*}{Method} & \multicolumn{8}{c|}{Effect   size against}             & \multicolumn{2}{c|}{MSMARCO}                        & \multicolumn{2}{c|}{BEIR} & \multirow{2}{*}{Lotte} \\ \cmidrule(l){3-14} 
                  &                         & \multicolumn{4}{c|}{PGT (d)} & \multicolumn{4}{c|}{SPLADE (b)} & \multicolumn{2}{c|}{Latency} & 18    & \textgreater{}1M &       \\
                  &                         & Mean   & +    & =   & -  & Mean   & +   & =    & -    & Average   & p99                      & \multicolumn{2}{c|}{AvG L}              & AvG L         \\ \midrule
\multicolumn{15}{c}{Baselines}   \\
\midrule 
a & BM25                & -9.6 & 1 & 6 & 23  & -11.2 & 1 & 6  & 23 & 1.0  & 1.0  & 1.0  & 1.0  & 1.0   \\
b & SPLADE (ours)              & 1.6 & 16 & 11  & 3 & \multicolumn{4}{c|}{N/A}    & 19.1 & 12.4 & 24.8 & 32.6 & 21.3 \\
\midrule 
\multicolumn{15}{c}{Advanced Baselines}   \\ \midrule 
c & (b) pruned to dataset original statistics       & -1.8 & 2 & 14 & 14 & -3.4 & 1 & 6 & 23 & 0.7  & 0.4  & 2.3  & 2.6  & 2.7   \\
d & \textbf{P}seudo-\textbf{G}uided \textbf{T}raversal ($a \xrightarrow{} b$)  & \multicolumn{4}{c|}{N/A} & -1.6 & 3 & 11 & 16 & 1.1  & 1.0  & 1.2  & 1.2  & 1.3 \\
\midrule 
\multicolumn{15}{c}{This work}   \\
\midrule 
e & Re-weighted documents of (c) with $k1=100$           & -4.9 & 1 & 4 & 25 & -6.5 & 1 & 3  & 26 & 0.5 & 0.3 & 1.1 & 1.2 & 1.4 \\
f & Two-Stage ($c \xrightarrow{} b$)      & 1.5 & 15 & 11  & 4 & -0.1  & 0 & 22 & 8 & 0.8 & 0.4 & 2.5 & 2.7 & 3.0 \\
g & Two-Stage ($e \xrightarrow{} b$) & 1.1 & 14 & 12  & 4 & -0.5  & 2 & 16 & 12 & 0.6 & 0.3 & 1.4 & 1.3 & 1.7 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/trec.tex <==
\begin{table}[ht]
\caption{Experiments on \car{document-centric} pruning of eff-V-L SPLADE on the TREC-DL queries (2019 and 2020). The $\times$ value represents the speedup compared to the baseline. $\dagger$ indicates statistical significance compared to the baseline.}
\label{tab:trec}
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{ccccccc}
\toprule
% \multirow{2}{*}{Min score}      & \multicolumn{3}{c|}{TREC-DL 2019}      & \multicolumn{3}{c}{TREC-DL 2020}   \\
% & Latency (x) & nDCG@10 & R@1k & Latency (x) & nDCG@10 & R@1k \\
Max size & \multicolumn{3}{c}{TREC-DL 2019}      & \multicolumn{3}{c}{TREC-DL 2020}   \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
 & Latency ($\times$) & nDCG@10 & R@1k & Latency (x) & nDCG@10 & R@1k \\
\midrule
\car{30 522}    & 28.2 (1.0$\times$) & 71.4 & 84.8 & 30.2 (1.0$\times$) & 71.5 & 86.2 \\
\midrule
\multicolumn{7}{c}{Prune by document size (D)} \\
\midrule
64        & 13.2 (2.1$\times$) & 69.3$^\dagger$ & 83.5$^\dagger$  & 13.7 (2.2$\times$) & 70.4 & 84.8$^\dagger$\\
32        & 8.8 (3.2$\times$)  & 67.9$^\dagger$ & 79.0$^\dagger$  & 8.9 (3.4$\times$) & 67.2$^\dagger$ & 81.8$^\dagger$\\
16         & 6.0 (4.7$\times$)  & 64.4$^\dagger$ & 74.6$^\dagger$  & 6.5 (4.6$\times$) & 65.0$^\dagger$ & 79.4$^\dagger$\\
8         & 3.4 (16.6$\times$) & 58.82$^\dagger$ & 67.0$^\dagger$  & 3.5 (8.6$\times$) & 59.5$^\dagger$ & 70.2$^\dagger$\\
4         & 1.7 (16.6$\times$) & 52.4$^\dagger$ & 54.5$^\dagger$  & 1.7 (17.8$\times$) & 48.6$^\dagger$ & 60.7$^\dagger$\\

\bottomrule
\end{tabular}
}
\end{table}

%1.7 60.69

%prune_size_8.0,prune_size_16.0,prune_size_32.0,prune_size_64.0,prune_size_128.0



==> tables/tripclick.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table}[ht]
\centering
\caption{
 Experiments on TripClick HEAD queries.$^\dagger$ indicates statistical significance difference compared to the baseline.% $*$ means no statistical difference with the non pruned version.
}
\adjustbox{max width=\columnwidth}{%
\begin{tabular}{c ccc ccc}
\toprule
%\textbf{\#}
\multirow{2}{*}{Max Size}   &    \multicolumn{3}{c}{Finetuning}      & \multicolumn{3}{c}{Zero-Shot}  \\
 \cmidrule(lr){2-4}\cmidrule(lr){5-7}
& Latency ($\times$)      
& MRR@10 
& R@1k   
& Latency ($\times$)      
& MRR@10 
& R@1k   \\ 
\midrule
\car{30 522}     & 5.8 (1.0$\times$) & 54.5 & \textbf{88.8} &  4.2 (1.0$\times$) & \textbf{32.0} & \textbf{83.6} \\
\midrule
\multicolumn{7}{c}{Prune by document size (D)} \\
\midrule

%a &
%basic &
%54.5$^{fg}$\hphantom{$^{bcde}$} &
%26.6$^{fg}$\hphantom{$^{bcde}$} &
%88.8$^{defg}$\hphantom{$^{bc}$} &
%\textbf{32.0}$^{efg}$\hphantom{$^{bcd}$} &
%\textbf{16.4}$^{defg}$\hphantom{$^{bc}$} &
%83.6$^{cdefg}$\hphantom{$^{b}$} \\
%b &

%128 &
%4.6 (1.3x) &
%56.3  & %$^{afg}$\hphantom{$^{cde}$} &
%\textbf{89.0} &%$^{cdefg}$\hphantom{$^{a}$} &
%3.99 (1.06x)  &
%32.0&%$^{efg}\hphantom{$^{acd}$} &
%\textbf{83.7}  \\ %$^{cdefg}$\hphantom{$^{a}$} \\
%%c &
64 &
 3.1 (1.9$\times$)  &
\textbf{56.7}$^\dagger$&%$^{aefg}$\hphantom{$^{bd}$} &
88.3$^\dagger$ &%$^{defg}$\hphantom{$^{ab}$} &
2.5  (1.7$\times$)  &
31.6\hphantom{$\dagger$}&%$^{efg}$\hphantom{$^{abd}$} &
82.8$^\dagger$ \\ %$^{defg}$\hphantom{$^{ab}$} \\
%d &
32 & 
1.9 (3.0$\times$) &
55.8\hphantom{$\dagger$}&%$^{fg}$\hphantom{$^{abce}$} &
86.8$^\dagger$ &%$^{efg}$\hphantom{$^{abc}$} &
 1.7  (2.5$\times$)  &
31.5\hphantom{$\dagger$}&%$^{fg}$\hphantom{$^{abce}$} &
80.1$^\dagger$ \\ %$^{efg}$\hphantom{$^{abc}$} \\
%e &
16 &
  1.2 (4.6$\times$)  &
54.7\hphantom{$\dagger$} &%$^{fg}$\hphantom{$^{abcd}$} &
83.4$^\dagger$ &%$^{fg}$\hphantom{$^{abcd}$} &
 1.1  (3.8$\times$) &
29.9$^\dagger$ &%$^{fg}$\hphantom{$^{abcd}$} &
73.4 $^\dagger$ \\ %$^{fg}$\hphantom{$^{abcd}$} \\
%f &
8 &
1.0 (5.8$\times$)   &
51.3$^\dagger$&%$^{g}$\hphantom{$^{abcde}$} &
76.8$^\dagger$ &%$^{g}$\hphantom{$^{abcde}$} &
1.0  (4.1$\times$)  &
27.7$^\dagger$  &%$^{g}$\hphantom{$^{abcde}$} &
58.9 $^\dagger$ \\%$^{g}$\hphantom{$^{abcde}$} \\
%g &
4 &
 1.0 (5.6$\times$)  &
42.9$^\dagger$ &%\hphantom{$^{abcdef}$} &
66.0$^\dagger$ &%\hphantom{$^{abcdef}$} &
0.8  (5.2$\times$)  &
22.5$^\dagger$ &%\hphantom{$^{abcdef}$} &
41.3$^\dagger$  \\ %\hphantom{$^{abcdef}$} \\
\bottomrule
\end{tabular}
}
\label{tab:tripclick}
\end{table}
\vspace{-0.5cm}

==> tikz/with_reranking/MSMARCO/figure.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{120px}{%
         \input{tikz/with_reranking/MSMARCO/legend.tex}}
%}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/with_reranking/MSMARCO/pisa.tex}
         }
     \end{subfigure}
      \caption{Two stage SPLADE over MSMARCO. With log on the xaxis}
     \label{fig:with_rerank_msmarco}
\end{figure*}





==> tikz/with_reranking/MSMARCO/figure2.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{120px}{%
         \input{tikz/with_reranking/MSMARCO/legend.tex}}
%}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/with_reranking/MSMARCO/pisa2.tex}
         }
     \end{subfigure}
      \caption{Two stage SPLADE over MSMARCO. Without log on the xaxis}
     \label{fig:with_rerank_msmarco_wout}
\end{figure*}





==> tikz/with_reranking/MSMARCO/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=3,
legend entries={
\textsc{Best},
\textsc{Rerank only},
\textsc{Rerank + load disk },
\textsc{Rerank top 100},
\textsc{Rerank top 250},
\textsc{Rerank top 1k},
\textsc{L SPLADE},
\textsc{Full SPLADE},
                        }]
         \addlegendimage{bestplot};
         \addlegendimage{edrerankplot};
         \addlegendimage{sdrerankplot};
         \addlegendimage{kcentplot};
         \addlegendimage{ktwofiveplot};
         \addlegendimage{k1kplot};         
         \addlegendimage{spladelexicalplot};
         \addlegendimage{spladeplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/with_reranking/MSMARCO/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel={Latency (PISA, in ms)},
           ylabel=MRR@10,
           ymin=0.28, ymax=0.4,
            xmode=log,
            log ticks with fixed point,log basis x={2},
            xmin=3.8,xmax=133,
            xtick={4,8,16,32,64,128},
                      xticklabels = {4,8,16,32,64,128}           
           ]
         \addplot[bestplot] table {tikz/with_reranking/MSMARCO/best.txt};
         \addplot[edrerankplot] table {tikz/with_reranking/MSMARCO/rerank_without_load.txt};
         \addplot[sdrerankplot] table {tikz/with_reranking/MSMARCO/rerank_with_load_disk.txt};
        \addplot[scatter, only marks,
          scatter/classes={30={mark=square*,\bestc, mark size=3pt},
                           32={mark=*,\bestc, mark size=3pt},
                           50={mark=pentagon*,\edc, mark size=3pt},
                           51={mark=oplus,\edc, mark size=3pt},
                           52={mark=x,\edc, mark size=3pt},                         
                           60={mark=pentagon*,\sdc, mark size=3pt},
                           61={mark=oplus,\sdc, mark size=3pt},
                           62={mark=x,\sdc, mark size=3pt},                        
                           70={mark=pentagon*,\effvc, mark size=3pt},
                           71={mark=oplus,\effvc, mark size=3pt},
                           72={mark=x,\effvc, mark size=3pt}                         
                          },
          scatter src=explicit symbolic  
          ] table[x index=0,y index=1,meta index=2] {tikz/with_reranking/MSMARCO/all.txt};
       \end{axis}
    \end{tikzpicture}


==> tikz/with_reranking/MSMARCO/pisa2.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel={Latency (PISA, in ms)},
           ylabel=MRR@10,
           ymin=0.28, ymax=0.4,
            xmin=0,xmax=133,
%            xtick={0,2,4,8,16,32,64,128},
%                      xticklabels = {4,8,16,32,64,128}           
           ]
         \addplot[bestplot] table {tikz/with_reranking/MSMARCO/best.txt};
         \addplot[edrerankplot] table {tikz/with_reranking/MSMARCO/rerank_without_load.txt};
         \addplot[sdrerankplot] table {tikz/with_reranking/MSMARCO/rerank_with_load_disk.txt};
        \addplot[scatter, only marks,
          scatter/classes={30={mark=square*,\bestc, mark size=3pt},
                           32={mark=*,\bestc, mark size=3pt},
                           50={mark=pentagon*,\edc, mark size=3pt},
                           51={mark=oplus,\edc, mark size=3pt},
                           52={mark=x,\edc, mark size=3pt},                         
                           60={mark=pentagon*,\sdc, mark size=3pt},
                           61={mark=oplus,\sdc, mark size=3pt},
                           62={mark=x,\sdc, mark size=3pt},                        
                           70={mark=pentagon*,\effvc, mark size=3pt},
                           71={mark=oplus,\effvc, mark size=3pt},
                           72={mark=x,\effvc, mark size=3pt}                         
                          },
          scatter src=explicit symbolic  
          ] table[x index=0,y index=1,meta index=2] {tikz/with_reranking/MSMARCO/all.txt};
       \end{axis}
    \end{tikzpicture}


==> tikz/with_reranking/MSMARCO_pruning/figure.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{120px}{%
         \input{tikz/with_reranking/MSMARCO_pruning/legend.tex}}
%}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/with_reranking/MSMARCO_pruning/pisa.tex}
         }
     \end{subfigure}
      \caption{Two stage SPLADE over MSMARCO. With log on the xaxis}
     \label{fig:with_rerank_msmarco}
\end{figure*}





==> tikz/with_reranking/MSMARCO_pruning/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=3,
legend entries={
\textsc{Best},
\textsc{Pruning},
\textsc{Pruning + Lexical Query},
\textsc{Rerank BEST},
\textsc{Rerank Pruning},
\textsc{Rerank Pruning + Lexical Query},
\textsc{L SPLADE},
\textsc{Full SPLADE}
                        }]
         \addlegendimage{bestplot};
         \addlegendimage{pruningplot};         
         \addlegendimage{pruninglexicalplot};         
         \addlegendimage{edrerankplot};
         \addlegendimage{rerankpruningplot};         
         \addlegendimage{rerankpruninglexicalplot};         
         \addlegendimage{spladelexicalplot};
         \addlegendimage{spladeplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/with_reranking/MSMARCO_pruning/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel={Latency (PISA, in ms)},
           ylabel=MRR@10,
           ymin=0, ymax=0.4,
            %xmode=log,
            %log ticks with fixed point,log basis x={2},
            xmin=0,xmax=32,
%            xtick={2,4,8,16,32},
%                      xticklabels = {2,4,8,16,32}           
           ]
         \addplot[bestplot] table {tikz/with_reranking/MSMARCO_pruning/best.txt};
         \addplot[edrerankplot] table {tikz/with_reranking/MSMARCO_pruning/rerank_lexical.txt};
         \addplot[pruningplot] table {tikz/with_reranking/MSMARCO_pruning/pruning.txt};
         \addplot[pruninglexicalplot] table {tikz/with_reranking/MSMARCO_pruning/pruning_lexical.txt};
         \addplot[rerankpruninglexicalplot] table {tikz/with_reranking/MSMARCO_pruning/rerank_lexical_pruning.txt};
         \addplot[rerankpruningplot] table {tikz/with_reranking/MSMARCO_pruning/rerank_pruning.txt};
        \addplot[scatter, only marks,
          scatter/classes={30={mark=square*,\bestc, mark size=3pt},
                           32={mark=*,\bestc, mark size=3pt},
                           50={mark=pentagon*,\edc, mark size=3pt},
                           51={mark=oplus,\edc, mark size=3pt},
                           52={mark=x,\edc, mark size=3pt},                         
                           60={mark=pentagon*,\sdc, mark size=3pt},
                           61={mark=oplus,\sdc, mark size=3pt},
                           62={mark=x,\sdc, mark size=3pt},                        
                           70={mark=pentagon*,\effvc, mark size=3pt},
                           71={mark=oplus,\effvc, mark size=3pt},
                           72={mark=x,\effvc, mark size=3pt}                         
                          },
          scatter src=explicit symbolic  
          ] table[x index=0,y index=1,meta index=2] {tikz/with_reranking/MSMARCO_pruning/all.txt};
       \end{axis}
    \end{tikzpicture}


==> tikz/without_reranking/BEIR/figure.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{120px}{%
         \input{tikz/without_reranking/BEIR/legend.tex}}
%}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/without_reranking/BEIR/pisa.tex}
         }
     \end{subfigure}
      \caption{Two stage SPLADE over BEIR (13 datasets), considering 0 latency for reranking and the latency of MSMARCO.}
     \label{fig:without_rerank_beir}
\end{figure*}





==> tikz/without_reranking/BEIR/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=4,
legend entries={
\textsc{ED},
\textsc{Rerank-ed},
\textsc{SD},
\textsc{Rerank-SD},
\textsc{Best},
\textsc{Rerank-BEST},
\textsc{Eff-V-Large},
\textsc{Rerank-Eff-V-Large},
\textsc{L SPLADE},
\textsc{QL SPLADE},
\textsc{Full SPLADE},
                        }]
         \addlegendimage{edplot};
         \addlegendimage{edrerankplot};
         \addlegendimage{sdplot};
         \addlegendimage{sdrerankplot};
         \addlegendimage{bestplot};
         \addlegendimage{bestrerankplot};
         \addlegendimage{effvplot};
         \addlegendimage{effvrerankplot};
         \addlegendimage{spladelexicalplot};
         \addlegendimage{spladeqlexicalplot};
         \addlegendimage{spladeplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/without_reranking/BEIR/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel={Latency MSMARCO (PISA, in ms)},
           ylabel=average nDCG@10 over 13 datasets,
           ymin=0.43, ymax=0.53,
            xmode=log,
            log ticks with fixed point,log basis x={2},
            xmin=3.8,xmax=512,
            xtick={4,8,16,32,64,128,256,512},
                      xticklabels = {4,8,16,32,64,128,256,512}           
           ]
         \addplot[edplot] table {tikz/without_reranking/BEIR/ed.txt};
         \addplot[edrerankplot] table {tikz/without_reranking/BEIR/ed_rerank.txt};
         \addplot[sdplot] table {tikz/without_reranking/BEIR/sd.txt};
         \addplot[sdrerankplot] table {tikz/without_reranking/BEIR/sd_rerank.txt};
         \addplot[bestplot] table {tikz/without_reranking/BEIR/best.txt};
         \addplot[bestrerankplot] table {tikz/without_reranking/BEIR/best_rerank.txt};
         \addplot[effvplot] table {tikz/without_reranking/BEIR/effv.txt};
         \addplot[effvrerankplot] table {tikz/without_reranking/BEIR/effv_rerank.txt};
        \addplot[scatter, only marks,
          scatter/classes={10={mark=square*,\edc, mark size=3pt},
                           11={mark=triangle*,\edc, mark size=3pt},
                           12={mark=*,\edc, mark size=3pt},
                           20={mark=square*,\sdc, mark size=3pt},
                           21={mark=triangle*,\sdc, mark size=3pt},
                           22={mark=*,\sdc, mark size=3pt},
                           30={mark=square*,\bestc, mark size=3pt},
                           31={mark=triangle*,\bestc, mark size=3pt},
                           32={mark=*,\bestc, mark size=3pt},
                           40={mark=square*,\effvc, mark size=3pt},
                           41={mark=triangle*,\effvc, mark size=3pt},
                           42={mark=*,\effvc, mark size=3pt}
                          },
          scatter src=explicit symbolic  
          ] table[x index=0,y index=1,meta index=2] {tikz/without_reranking/BEIR/all.txt};
       \end{axis}
    \end{tikzpicture}


==> tikz/without_reranking/MSMARCO/figure.tex <==
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
\adjustbox{max width=\textwidth}{%
%         \raisebox{120px}{%
         \input{tikz/without_reranking/MSMARCO/legend.tex}}
%}
     \end{subfigure}
     \begin{subfigure}[t]{0.3\textwidth}


         \centering
\adjustbox{max width=\textwidth}{%
         \input{tikz/without_reranking/MSMARCO/pisa.tex}
         }
     \end{subfigure}
      \caption{Two stage SPLADE over MSMARCO, considering 0 latency for reranking.}
     \label{fig:without_rerank_msmarco}
\end{figure*}





==> tikz/without_reranking/MSMARCO/legend.tex <==
\begin{tikzpicture}
\begin{customlegend}[
legend columns=4,
legend entries={
\textsc{ED},
\textsc{Rerank-ed},
\textsc{SD},
\textsc{Rerank-SD},
\textsc{Best},
\textsc{Rerank-BEST},
\textsc{Eff-V-Large},
\textsc{Rerank-Eff-V-Large},
\textsc{L SPLADE},
\textsc{QL SPLADE},
\textsc{Full SPLADE},
                        }]
         \addlegendimage{edplot};
         \addlegendimage{edrerankplot};
         \addlegendimage{sdplot};
         \addlegendimage{sdrerankplot};
         \addlegendimage{bestplot};
         \addlegendimage{bestrerankplot};
         \addlegendimage{effvplot};
         \addlegendimage{effvrerankplot};
         \addlegendimage{spladelexicalplot};
         \addlegendimage{spladeqlexicalplot};
         \addlegendimage{spladeplot};
        \end{customlegend}
\end{tikzpicture}


==> tikz/without_reranking/MSMARCO/pisa.tex <==
   \begin{tikzpicture}
       \begin{axis}[
           xlabel={Latency (PISA, in ms)},
           ylabel=MRR@10,
           ymin=0.28, ymax=0.4,
            xmode=log,
            log ticks with fixed point,log basis x={2},
            xmin=3.8,xmax=512,
            xtick={4,8,16,32,64,128,256,512},
                      xticklabels = {4,8,16,32,64,128,256,512}           
           ]
         \addplot[edplot] table {tikz/without_reranking/MSMARCO/ed.txt};
         \addplot[edrerankplot] table {tikz/without_reranking/MSMARCO/ed_rerank.txt};
         \addplot[sdplot] table {tikz/without_reranking/MSMARCO/sd.txt};
         \addplot[sdrerankplot] table {tikz/without_reranking/MSMARCO/sd_rerank.txt};
         \addplot[bestplot] table {tikz/without_reranking/MSMARCO/best.txt};
         \addplot[bestrerankplot] table {tikz/without_reranking/MSMARCO/best_rerank.txt};
         \addplot[effvplot] table {tikz/without_reranking/MSMARCO/effv.txt};
         \addplot[effvrerankplot] table {tikz/without_reranking/MSMARCO/effv_rerank.txt};
        \addplot[scatter, only marks,
          scatter/classes={10={mark=square*,\edc, mark size=3pt},
                           11={mark=triangle*,\edc, mark size=3pt},
                           12={mark=*,\edc, mark size=3pt},
                           20={mark=square*,\sdc, mark size=3pt},
                           21={mark=triangle*,\sdc, mark size=3pt},
                           22={mark=*,\sdc, mark size=3pt},
                           30={mark=square*,\bestc, mark size=3pt},
                           31={mark=triangle*,\bestc, mark size=3pt},
                           32={mark=*,\bestc, mark size=3pt},
                           40={mark=square*,\effvc, mark size=3pt},
                           41={mark=triangle*,\effvc, mark size=3pt},
                           42={mark=*,\effvc, mark size=3pt}
                          },
          scatter src=explicit symbolic  
          ] table[x index=0,y index=1,meta index=2] {tikz/without_reranking/MSMARCO/all.txt};
       \end{axis}
    \end{tikzpicture}

